Robust Computation of Dipole Electromagnetic Fields in Arbitrarily-Anisotropic, Planar-Stratified Environments

We develop a general-purpose formulation, based on two-dimensional spectral integrals, for computing electromagnetic fields produced by arbitrarily-oriented dipoles in planar-stratified environments, where each layer may exhibit arbitrary and independent anisotropy in both the (complex) permittivity and permeability. Among the salient features of our formulation are (1) computation of eigenmodes (characteristic plane waves) supported in arbitrarily anisotropic media in a numerically robust fashion, (2) implementation of an hp-adaptive refinement for the numerical integration to evaluate the radiation and weakly-evanescent spectra contributions, and (3) development of an adaptive extension of an integral convergence acceleration technique to compute the strongly-evanescent spectrum contribution. While other semianalytic techniques exist to solve this problem, none have full applicability to media exhibiting arbitrary double anisotropies in each layer, where one must account for the whole range of possible phenomena such as mode coupling at interfaces and non-reciprocal mode propagation. Brute-force numerical methods can tackle this problem but only at a much higher computational cost. The present formulation provides an efficient and robust technique for field computation in arbitrary planar-stratified environments. We demonstrate the formulation for a number of problems related to geophysical exploration.

==> url.tex <==
 url.sty  ver 3.3    12-Apr-2006   Donald Arseneau   asnd@triumf.ca
% Copyright 1996-2006 Donald Arseneau,  Vancouver, Canada.
% This program can be used, distributed, and modified under the terms
% of the LaTeX Project Public License.
%
% A form of \verb that allows linebreaks at certain characters or
% combinations of characters, accepts reconfiguration, and can usually
% be used in the argument to another command.  It is intended for email
% addresses, hypertext links, directories/paths, etc., which normally
% have no spaces.  The font may be selected using the \urlstyle command,
% and new url-like commands can be defined using \urldef.
%
% Usage:    Conditions:
% \url{ }   If the argument contains any "%" or "^^", or ends with
%           "\", it can't be used in the argument to another command.
%           The argument must not contain unbalanced braces.
% \url|  |  ...where "|" is any character not used in the argument and not
%           "{" or a space.  The same restrictions as above except that the
%           argument may contain unbalanced braces.
% \urldef\xyz\url{ }
% \xyz      a defined-url: "\xyz" can be used anywhere, no matter what
%           characters it contains.
% \DeclareUrlCommand\abc{settings}: makes \abc{ } like \url{ }
%
% See further instructions after "\endinput"
%

% default style assignments
\def\UrlBreaks{\do\.\do\@\do\\\do\/\do\!\do\_\do\|\do\;\do\>\do\]%
 \do\)\do\,\do\?\do\'\do+\do\=\do\#}%
\def\UrlBigBreaks{\do\:\do@url@hyp}%
\def\UrlNoBreaks{\do\(\do\[\do\{\do\<}%
% any ordinary characters that aren't usually:
\def\UrlOrds{\do\*\do\-\do\~\do\'\do\"\do\-}%
\def\UrlSpecials{\do\ {\Url@space}\do\%{\Url@percent}\do\^^M{\Url@space}%
   \Url@force@Tilde}% package option may force faked text-ascii-tilde

\@namedef{Url@OT1encSpecials}{%
  %  *Some* latin-1 or windows characters that ot1 has elsewhere:  OE  oe  ss
  \do\^^8c{\mathchar30 }\do\^^9c{\mathchar27 }\do\^^df{\mathchar25 }%
  \do\~{\lower.45ex\hbox{\m@th$\mathchar126$}}% For tt style
  % lots more to add, but I should later link into inputenc
  \do\^^b5{\mu}%
  \Url@OTnonTT % more for any but typewriter
  }

\def\Url@OTnonTT{\do\<{\langle}\do\>{\mathbin{\rangle}}\do
  \_{\_\penalty\@m}\do\|{\mid}\do\{{\lbrace}\do\}{\mathbin{\rbrace}}\do
  \\{\mathbin{\backslash}}\UrlTildeSpecial}

% *Some* latin-1 or windows characters. Most will pass through safely to T1 enc
% mu  inverted-?  OE  oe
% lots more to add, but I should later link into inputenc
\@namedef{Url@T1encSpecials}{\do\^^b5{\mu}\do\^^bf{\mathchar190 }%
  \do\^^8c{\mathchar215 }\do\^^9c{\mathchar247 }\do\^^df{\mathchar255 }%
  \do\^^ff{\mathchar184 }}

\@namedef{Url@LY1encSpecials}{\do\~{\mathchar158 }}

\def\UrlTildeSpecial{\do\~{\raise.45ex\hbox{\m@th$\scriptstyle\sim$}}}
\let\Url@force@Tilde\relax

\def\url@ttstyle{%
 \@ifundefined{selectfont}{\def\UrlFont{\tt}}{\def\UrlFont{\ttfamily}}}

\def\url@rmstyle{%
 \@ifundefined{selectfont}{\def\UrlFont{\rm}}{\def\UrlFont{\rmfamily}}}

\def\url@sfstyle{%
 \@ifundefined{selectfont}{\def\UrlFont{\sf}}{\def\UrlFont{\sffamily}}}

\def\url@samestyle{\def\UrlFont{}}

\@ifundefined{strip@prefix}{\def\strip@prefix#1>{}}{}
\@ifundefined{verbatim@nolig@list}{\def\verbatim@nolig@list{\do\`}}{}

% \Url sets up the reading the argument verbatim if possible
\def\Url{%
 \Url@movingtest
 \ifmmode\@nomatherr$\fi %$
 \let\do\@makeother \dospecials % verbatim catcodes
 \catcode`{\@ne \catcode`}\tw@ % with exceptions
 \catcode`\ =10 % allow "\url {x}"
 \catcode`\#=6  % always # -> ##, so I can later convert ## -> #
 \@ifnextchar\bgroup{\obeyspaces\obeylines\Url@z}\Url@y}

% \Url@y read arguments delimited like |...|, passing to \Url@z
\def\Url@y#1{\catcode`{11 \catcode`}11\obeyspaces\obeylines
  \def\@tempa##1#1{\Url@z{##1}}\@tempa}

% \Url@z read arguments delimited like {...}, verbatimizes with \meaning,
% performs character translations, then invokes the formatter.
\def\Url@z#1{\toks@{#1}\edef\Url@String{\the\toks@}%
  \edef\Url@String{\expandafter\strip@prefix\meaning\Url@String}%
%\if\urldebug \message{------------------------------------------------------}%
%\message{ \Url@String}\fi
% \meaning introduces spurious spaces in the text, so it would be nice
% to preserve the real spaces before \meaning, but that doesn't work --
% we can only do replacement on streams of non-syntactic characters.
  \Url@ObeySp % may be no-op; otherwise put ordinary (12) space characters
%\if\urldebug \message{ \Url@String}\fi
% we left the catcode of # with its normal value (6) so \meaning
% doubles it to ##.  Now we convert back to single #.  This allows
% \url{#} to appear in the arguments of other commands, where we can't
% make # be an ordinary character.  We make the single # active rather
% than `other' to support hyperref.sty.
  \Url@acthash
%\if\urldebug \message{ \Url@String}\fi
% Also make % active to support hyperref.
  \Url@actpercent
% now do any hyper referencing due to hyperref (or perform a url-def)
  \Url@HyperHook
% Now do the formatting in a group (can also have \Url@HyperHook take
% this as an argument.
  {\Url@FormatString}%
  \endgroup}

\let\Url@ObeySp\@empty
\let\UrlRight\@empty
\let\UrlLeft\@empty
\let\Url@HyperHook\@empty

% This is the normal way to format the strings, using math mode.
\def\Url@FormatString{%
 \UrlFont \Url@MathSetup
 $\fam\z@ \textfont\z@\font
 \expandafter\UrlLeft\Url@String\UrlRight
 \m@th$%
% \if\urldebug \showlists \fi
}%

\def\Url@MathSetup{%
 \medmuskip\Urlmuskip \thickmuskip\medmuskip \thinmuskip0mu%
 \relpenalty\UrlBigBreakPenalty \binoppenalty\UrlBreakPenalty
 \expandafter\let\expandafter\UrlEncSpecials\csname Url@\f@encoding encSpecials\endcsname
 % Insert test for unknown encodings here \ifx\UrlEncSpecials\relax
 \ifdim\fontdimen\thr@@\font=\z@ \let\Url@OTnonTT\relax \fi
 \@tempcnta\z@ %  \fam\multiply\@tempcnta\@cclvi
 \let\do\set@mathcode \UrlOrds % ordinary characters that were special
 \advance\@tempcnta 8192 \UrlBreaks % bin
 \advance\@tempcnta 4096 \UrlBigBreaks % rel
 \advance\@tempcnta 4096 \UrlNoBreaks % open
 \let\do\set@mathact \UrlSpecials \UrlEncSpecials % active
 \let\do\set@mathnolig \verbatim@nolig@list % prevent ligatures
}

\def\set@mathcode#1{\count@`#1\advance\count@\@tempcnta
%\message{Set mathcode of \string #1 (\number`#1) = \number`#1 + \number\@tempcnta. }%
\mathcode`#1\count@}
\def\set@mathact#1#2{\mathcode`#1=32768 \begingroup
    \lccode`\~`#1\lowercase{\endgroup\def~}{#2}}
\def\set@mathnolig#1{\ifnum\mathcode`#1<32768
   \begingroup\lccode`\~`#1\lowercase{\endgroup
     \edef~}{\mathchar\number\mathcode`#1_{\/}}%
   \mathcode`#1=32768 \fi}

\def\Url@movingtest{\begingroup
 \ifx\let\HyPsd@LetCommand % we are already in a pdf string!
  \expandafter\Url@unmove \fi % give the argument and hope for the best
 \let\Url@moving\relax\relax\relax
 \ifx\Url@moving\relax\else \expandafter\Url@unmove \fi
 \endgroup}
\long\def\Url@unmove#1\Url@y{\endgroup \ifx\protect\relax\else\protect\Url\fi}
\edef\Url@moving{\csname Url Error\endcsname}
\expandafter\edef\Url@moving
 {\csname url used in a moving argument.\endcsname}
\expandafter\expandafter\expandafter \let \Url@moving\@undefined

\def\urldef#1#2{\begingroup \setbox\z@\hbox\bgroup
  \def\Url@HyperHook##1\endgroup{\Url@def{#1}{#2}}%
  % Because hyperref breaks \urldef and does not define its own (Grrrr!)...
  \def\url@##1{\egroup\endgroup\DeclareRobustCommand#1{#2{##1}}}%
 #2}
\def\Url@def#1#2{%
   \toks0\expandafter{\Url@String}%
   \protected@edef\Url@String{\Url@String}%
   \toks1\expandafter{\Url@String}%
   \edef\Url@String{\endgroup\egroup\endgroup\def
     \expandafter\noexpand\csname\expandafter\@gobble\string#1 \endcsname
     {\noexpand\Url@eitherdef{\the\toks1}{\noexpand#2{\the\toks0}}}}%
   \Url@String
   \edef#1{\noexpand\protect
      \expandafter\noexpand\csname\expandafter\@gobble\string#1 \endcsname}%
  }
\def\Url@eitherdef{\ifx\let\HyPsd@LetCommand % we are already in a pdf string!
  \expandafter\@firstoftwo \else \expandafter\@secondoftwo \fi}

\def\urlstyle#1{\expandafter\protect\csname url@#1style\endcsname}

\def\DeclareUrlCommand#1#2{\def#1{\leavevmode\begingroup #2\Url}}

% Sample (and default) configuration:
%
\DeclareUrlCommand\url{}
\urlstyle{tt}
%
\newmuskip\Urlmuskip \Urlmuskip=0mu
\mathchardef\UrlBreakPenalty=\binoppenalty
\mathchardef\UrlBigBreakPenalty=\relpenalty
%
% picTeX defines \path, so declare it optionally:
\@ifundefined{path}{\DeclareUrlCommand\path{\urlstyle{tt}}}{}
%
% too many styles define \email like \address, so I will not define it.
% \DeclareUrlCommand\email{\urlstyle{rm}}

% Process LaTeX \package options
%
\let\Url@sppen\@M
\def\Url@space{\penalty\Url@sppen}
\def\do@url@hyp{}% by default, no breaks after hyphens

\@ifundefined{ProvidesPackage}{
}{\ProvidesPackage
 {url}[2006/04/12 \space ver 3.3 \space Verb mode for urls, etc.]
\DeclareOption{hyphens}{\def\do@url@hyp{\do\-}}% allow breaks after hyphens
\DeclareOption{obeyspaces}{\let\Url@ObeySp\relax}% a flag for later
\DeclareOption{spaces}{\def\Url@sppen{\UrlBreakPenalty}}
\DeclareOption{LY1}{}
\DeclareOption{T1}{}
\DeclareOption{allowmove}{\let\Url@moving\@empty}
\DeclareOption{lowtilde}{%
  \def\UrlTildeSpecial{\do\~{\raise.2ex\hbox{\m@th$\scriptstyle\sim$}}}
  \let\Url@force@Tilde\UrlTildeSpecial
}
\ProcessOptions\relax
\ifx\Url@ObeySp\relax % [obeyspaces] was declared
  \begingroup \lccode`+=32 \lowercase
   {\endgroup \def\Url@ObeySp{\Url@Edit\Url@String{ }{+}}}
   \def\Url@space{\penalty\Url@sppen\ }
\fi
}
\ifx\f@encoding\undefined \def\f@encoding{OT1}\fi

\begingroup
% \Url@acthash:    convert `other' (doubled) ## to active #
% \Url@actpercent: convert `other' % to active %
 \lccode`+=`\# \lccode`\~=`\#
  \lowercase {\long\gdef\Url@acthash{\Url@Edit\Url@String{++}{~}%
     \ifnum\mathcode`\#<32768 \def~{\#}\fi}}%
 \lccode`+=`\% \lccode`\~=`\%
  \lowercase {\long\gdef\Url@actpercent{\Url@Edit\Url@String{+}{~}%
    \ifnum\mathcode`\%<32768 \def~{\%}\fi}}%
 \catcode13=12 %
 \gdef\Url@percent{\@ifnextchar^^M{\@gobble}{\mathbin{\mathchar`\%}}}%
\endgroup%

%   Edit macro #1 changing all appearances of pattern #2 to replacement #3.
%   The replacement is recursive, so don't put the search pattern into the
%   replacement text!

{ \catcode`Q=3

\gdef\Url@Edit#1#2#3{%
 \begingroup % \tracingall
 \def\DOE@a{\endgroup\def#1}% Just so I can \expandafter it safely.
 \def\DOE@b##1#2##2Q##3{\@ifblank{##2}% if finished,
   {\DOE@c ##1Q}% then remove \@empty's and redefine macro
   {\DOE@b##1##3##2Q{##3}}% else, re-iterate
 }%  the leading \@empty preserves braces, as does the trailing pattern:
 \expandafter\DOE@b\expandafter\@empty #1\@empty#2Q{#3}}
\gdef\DOE@c#1\@empty Q{\expandafter\DOE@a\expandafter{#1}}
%
%  \@ifblank (LaTeX syntax) --- checks if parameter is blank (Spaces
%     count as blank) use \@ifblank{#1}{true case}{false case} etc
\long\gdef\@ifblank#1{\@Ifbl@nk#1QQ\@secondoftwo\@firstoftwo!}%
\long\gdef\@Ifbl@nk#1#2Q#3#4#5!{#4}

} % restore Q catcode


%\ifx\urldebug\@undefined \def\urldebug{01}\fi

\endinput
%
% url.sty  ver 3.3    12-Apr-2006   Donald Arseneau   asnd@triumf.ca
%
% This package defines "\url", a form of "\verb" that allows linebreaks,
% and can often be used in the argument to another command.  It can be
% configured to print in different formats, and is particularly useful for
% hypertext links, email addresses, directories/paths, etc.  The font may
% be selected using the "\urlstyle" command and pre-defined text can be
% stored with the "\urldef" command. New url-like commands can be defined,
% and a "\path" command is provided this way.
%
% Usage:    Conditions:
% \url{ }   If the argument contains any "%", "#", or "^^", or ends with
%           "\", it can't be used in the argument to another command.
%           The argument must not contain unbalanced braces.
% \url|  |  ...where "|" is any character not used in the argument and not
%           "{" or a space.  The same restrictions as above except that the
%           argument may contain unbalanced braces.
% \xyz      for "\xyz" a defined-url;  this can be used anywhere, no matter
%           what characters it contains.
%
% The "\url" command is fragile, and its argument is likely to be very
% fragile, but a defined-url is robust.
%
% Package Option:  obeyspaces
% Ordinarily, all spaces are ignored in the url-text.  The "[obeyspaces]"
% option allows spaces, but may introduce spurious spaces when a url
% containing "\" characters is given in the argument to another command.
% So if you need to obey spaces you can say "\usepackage[obeyspaces]{url}",
% and if you need both spaces and backslashes, use a `defined-url' for
% anything with "\".
%
% Package Option:  hyphens
% Ordinarily, breaks are not allowed after "-" characters because this
% leads to confusion. (Is the "-" part of the address or just a hyphen?)
% The package option "[hyphens]" allows breaks after explicit hyphen
% characters.  The "\url" command will *never ever* hyphenate words.
%
% Package Option:  spaces
% Likewise, breaks are not usually allowed after spaces under the
% "[obeyspaces]" option, but giving the options "[obeyspaces,spaces]"
% will allow breaks at those spaces. (Note that it seems logical to
% allow the sole option "[spaces]" to let input spaces indicate break
% points, but not to display them in the output. This would be easy to
% implement, but is left out to avoid(?) confusion.)
%
% Package Option:  lowtilde
% Normal treatment of the ~ character is to use the font's "\textasciitilde"
% character, if it has one (or claims to).  Otherwise, the character is
% faked using a mathematic "\sim".  The "[lowtilde]" option causes a
% faked character to be used always (and a bit lower than usual).
%
% Defining a defined-url:
% Take for example the email address "myself%node@gateway.net" which could
% not be given (using "\url" or "\verb") in a caption or parbox due to the
% percent sign.  This address can be predefined with
%    \urldef{\myself}\url{myself%node@gateway.net}   or
%    \urldef{\myself}\url|myself%node@gateway.net|
% and then you may use "\myself" instead of "\url{myself%node@gateway.net}"
% in an argument, and even in a moving argument like a caption because a
% defined-url is robust.
%
% Style:
% You can switch the style of printing using "\urlstyle{tt}", where "tt"
% can be any defined style.  The pre-defined styles are "tt", "rm", "sf",
% and "same" which all allow the same linebreaks but different fonts --
% the first three select a specific font and the "same" style uses the
% current text font.  You can define your own styles with different fonts
% and/or line-breaking by following the explanations below.  The "\url"
% command follows whatever the currently-set style dictates.
%
% Alternate commands:
% It may be desireable to have different things treated differently, each
% in a predefined style; e.g., if you want directory paths to always be
% in typewriter and email addresses to be roman, then you would define new
% url-like commands as follows:
%
%    \DeclareUrlCommand\email{\urlstyle{rm}}
%    \DeclareUrlCommand\directory{\urlstyle{tt}}
%
% In fact, the "\directory" example is exactly the "\path" definition which
% is pre-defined in the package.  If you look above, you will see that "\url"
% is defined with
%    \DeclareUrlCommand\url{}
% I.e., using whatever "\urlstyle" and other settings are already in effect.
%
% You can make a defined-url for these other styles, using the usual
% "\urldef" command as in this example:
%
%    \urldef{\myself}{\email}{myself%node.domain@gateway.net}
%
% which makes "\myself" act like "\email{myself%node.domain@gateway.net}",
% if the "\email" command is defined as above.  The "\myself" command
% would then be robust.
%
% Defining styles:
% Before describing how to customize the printing style, it is best to
% mention something about the unusual implementation of "\url".  Although
% the material is textual in nature, and the font specification required
% is a text-font command, the text is actually typeset in *math* mode.
% This allows the context-sensitive linebreaking, but also accounts for
% the default behavior of ignoring spaces.  Now on to defining styles.
%
% To change the font or the list of characters that allow linebreaks, you
% could redefine the commands "\UrlFont", "\UrlBreaks", "\UrlSpecials" etc.
% directly in the document, but it is better to define a new `url-style'
% (following the example of "\url@ttstyle" and "\url@rmstyle") which defines
% all of "\UrlBigbreaks", "\UrlNoBreaks", "\UrlBreaks", "\UrlSpecials", and
% "\UrlFont".
%
% Changing font:
% The "\UrlFont" command selects the font.  The definition of "\UrlFont"
% done by the pre-defined styles varies to cope with a variety of LaTeX
% font selection schemes, but it could be as simple as "\def\UrlFont{\tt}".
% Depending on the font selected, some characters may need to be defined
% in the "\UrlSpecials" list because many fonts don't contain all the
% standard input characters.
%
% Changing linebreaks:
% The list of characters that allow line-breaks is given by "\UrlBreaks"
% and "\UrlBigBreaks", which have the format "\do\c" for character "c".
% The differences are that `BigBreaks' usually have a lower penalty and have
% different breakpoints when in sequence (as in "http://"): `BigBreaks'
% are treated as mathrels while `Breaks' are mathbins (see The TeXbook,
% p.170). In particular, a series of `BigBreak' characters will break at
% the end and only at the end; a series of `Break' characters will break
% after the first and after every following *pair*; there will be no
% break after a `Break' character if a `BigBreak' follows.  In the case
% of "http://" it doesn't matter whether ":" is a `Break' or `BigBreak' --
% the breaks are the same in either case; but for DECnet nodes with "::"
% it is important to prevent breaks *between* the colons, and that is why
% colons are `BigBreaks'.
%
% It is possible for characters to prevent breaks after the next following
% character (I use this for parentheses).  Specify these in "\UrlNoBreaks".
%
% You can do arbitrarily complex things with characters by making them
% active in math mode (mathcode hex-8000) and specifying the definition(s)
% in "\UrlSpecials".  This is used in the rm and sf styles for OT1 font
% encoding to handle several characters that are not present in those
% computer-modern style fonts.  See the definition of "\Url@do", which
% is used by both "\url@rmstyle" and "\url@sfstyle"; it handles missing
% characters via "\UrlSpecials".  The nominal format for setting each
% special character "c" is: "\do\c{<definition>}", but you can include
% other definitions too.
%
% If all this sounds confusing ... well, it is!  But I hope you won't need
% to redefine breakpoints -- the default assignments seem to work well for
% a wide variety of applications.  If you do need to make changes, you can
% test for breakpoints using regular math mode and the characters "+=(a".
%
% You can allow some spacing around the breakable characters by assigning
%    \Urlmuskip = 0mu plus 1mu
% You can change the penalties used for BigBreaks and Breaks by assigning
%    \mathchardef\UrlBreakPenalty=100 \mathchardef\UrlBigBreakPenalty=100
% The default penalties are "\binoppenalty" and "\relpenalty".  These have
% such odd non-LaTeX syntax because I don't expect people to need to
% change them often.
%
% Yet more flexibility:
% You can also customize the verbatim text by defining "\UrlRight" and/or
% "\UrlLeft", e.g., for ISO formatting of urls surrounded by "<  >", define
%
%    \DeclareUrlCommand\url{\def\UrlLeft{<url:\ }\def\UrlRight{>}%
%        \urlstyle{tt}}
%
% The meanings of "\UrlLeft" and "\UrlRight" are *not* reproduced verbatim.
% This lets you use formatting commands there, but you must be careful not
% to use TeX's special characters ("\^_%~#$&{}" etc.) improperly.
% You can also define "\UrlLeft" to reprocess the verbatim text, but the
% format of the definition is special:
%
%    \def\UrlLeft#1\UrlRight{ ... do things with #1 ... }
%
% Yes, that is "#1" followed by "\UrlRight" then the definition.  For
% example, to put a hyperTeX hypertext link in the DVI file:
%
%    \def\UrlLeft#1\UrlRight{\special{html:<a href="#1">}#1\special{html:</a>}}
%
% Using this technique, url.sty can provide a convenient interface for
% performing various operations on verbatim text.  You don't even need
% to print out the argument!  For greatest efficiency in such obscure
% applications, you can define a null url-style where all the lists like
% "\UrlBreaks" are empty.
%
% Revision History:
% ver 1.1 6-Feb-1996:
% Fix hyphens that wouldn't break and ligatures that weren't suppressed.
% ver 1.2 19-Oct-1996:
% Package option for T1 encoding; Hooks: "\UrlLeft" and "\UrlRight".
% ver 1.3 21-Jul-1997:
% Prohibit spaces as delimiter characters; change ascii tilde in OT1.
% ver 1.4 02-Mar-1999:
% LaTeX license; moving-argument-error
% ver 1.5 28-Mar-1999:
% possibility of spacing around break characters; re-settable penalties
% ver 1.6 20-Jun-2002:
% un-double #, fix obeyed-spaces, ignore trailing %, hook for hyperref
% (\Url@HyperHook), no macros in pre-processed url string (in \Url@String),
% limit catcode change of ~.
% ver 3.0 June 2003/Nov 2003:
% \DeclareUrlCommand; make font encoding automatic (only a few inputenc characters
% are supported yet - needs refactoring); reverse penalties.
% ver 3.1 Mar 2004:
% Remove spurious spaces in \url@XXstyle commands.
% ver 3.2 June 2005:
% Fix cmsy-symbols in tt bug (from 3.0); LY1 encoding bug; Enable plain
% with miniltx (again); Define the \urldef for hyperref; Lower "sim" tilde
% a little; fix \lowercase error in \UrlSpecials handling.
% ver 3.3 April 2006:
% Fix some encoding bugs and remove 8-bit characters.  lowtilde option
% The End

Test file integrity:  ASCII 32-57, 58-126:  !"#$%&'()*+,-./0123456789
:;<=>?@ABCDEFGHIJKLMNOPQRSTUVWXYZ[\]^_`abcdefghijklmnopqrstuvwxyz{|}~

